Dynamic Collective Choice: Social Optima

We consider a dynamic collective choice problem where a large number of players are cooperatively choosing between multiple destinations while being influenced by the behavior of the group. For example, in a robotic swarm exploring a new environment, a robot might have to choose between multiple sites to visit, but at the same time it should remain close to the group to achieve some coordinated tasks. We show that to find a social optimum for our problem, one needs to solve a set of Linear Quadratic Regulator problems, whose number increases exponentially with the size of the population. Alternatively, we develop via the Mean Field Games methodology a set of decentralized strategies that are independent of the size of the population. When the number of agents is sufficiently large, these strategies qualify as approximately socially optimal. To compute the approximate social optimum, each player needs to know its own state and the statistical distributions of the players' initial states and problem parameters. Finally, we give a numerical example where the cooperative and noncooperative cases have opposite behaviors. Whereas in the former the size of the majority increases with the social effect, in the latter, the existence of a majority is disadvantaged.

==> Nonuniform.tex <==
\section{Decentralized Pareto strategies - Nonuniform Weights}

In the previous sections, we consider 
the problem of finding one Pareto 
optimum by minimizing a social cost
whereby the players are uniformly 
penalized. By assigning, in the
social cost, nonuniform weights to the 
individual costs
one can compute a larger
number of Pareto Optima.
In fact the minima of the 
nonuniform social costs 
$\sum_{i=1}^N \alpha_i J_i(u_i,x^{(N)})$,
for $\alpha_i>0$, are Pareto Optima
with respect to the costs (\ref{eq-cost}).
Thus, we consider the problem of 
minimizing the following nonuniform 
social cost
\begin{equation} \label{nonuniform-cost}
J_{socn}(u,x^{(N)})=
\sum_{i=1}^N \alpha_i J_i(u_i,x^{(N)})
\end{equation}
Moreover, we consider nonuniform dynamics
\begin{align} \label{nonuniform-dynamic}
\dot{x}_i=A_i x_i + B_i u_i && 
i=1,\dots,N
\end{align}

We assume that the weights $\alpha_i$
are i.i.d. in a compact set 
$E \subset \mathbb{R}_{+*}$ and the 
dynamic parameters 
$\theta_i=(A_i,B_i)$ are i.i.d.
in a compact set $\Theta$. 
Moreover, we assume that the initial
conditions, the dynamic parameters and
the weights are independent. 
Let us denote the empirical measures 
of these parameters and weights 
$P^N_\theta(\mathcal A) = 1/N 
\sum_{i=1}^N 1_{\{\theta_i \in \mathcal A\}}$ 
and $P^N_\alpha(\mathcal A) = 
1/N \sum_{i=1}^N 1_{\{\alpha_i \in \mathcal A\}}$,
 for 
all (Borel) measurable sets $\mathcal A$. 
We assume that $P^N_\theta$ and $P^N_\alpha$ 
have weak limits $P_\theta$ 
and $P_\alpha$, that is, $\lim_{N\to\infty} 
\int_{\Theta} \phi (x) \mathrm{d}P^N_\theta(x)=
\int_{\Theta} \phi (x) \mathrm{d}P_\theta(x)$ 
and $\lim_{N\to\infty} \int_{E} \psi (x) 
\mathrm{d}P^N_\alpha(x)
=\int_{E} \psi (x) \mathrm{d}P_\alpha(x)$ 
for all $\phi$ and $\psi$ continuous. 
For further discussions about this 
assumption, one can refer 
to \cite{huang2012social}.
We seek a decentralized Pareto optimum where 
each agent knows its own
initial state, weight, dynamic 
parameters and the statistical distributions 
of the initial states, weights and dynamic 
parameters.

As in paragraph 
\ref{reduced-problem}, one can decompose
the social cost and prove that 
\[
\argmin_{u_i \in U} J_{socn}(u_i,u_{-i}^*)= 
\argmin_{u_i \in U} J_{socn,i}^{ind}
(u_i,{x^*_{-i}}^{(N)})
u_i^*
\] 
where $(u_i^*,u_{-i}^*)$ is the optimal control
law of $J_{socn}$,
\begin{multline*}
J_{socn,i}^{ind}(u_i,x^{(N)}_{-i})=\\
\mathbb{E} \Bigg ( \int_0^T \bigg\{ x_i^T\hat{Q}_i
x_i - q\alpha_i(x^{(N)}_{-i})^T \gamma^T (I_n-
\frac{\gamma}{N}) x_i\\
-\frac{q}{N} \sum_{j=1,j\neq i}
\alpha_j x_j^T \gamma x_i 
+\frac{q}{N} \sum_{j=1,j\neq i}
\alpha_j  (x^{(N)}_{-i})^T \gamma^T \gamma x_i\\ 
+ \frac{\alpha_ir}{2} \|u_i\|^2 \bigg\}
\mathrm{dt} 
+\frac{\alpha_iM}{2} \min
\limits_{j=1,\dots,l}\|x_i(T)-p_j\|^2 \Bigg ) 
\end{multline*}
\begin{equation*}
\hat{Q}_i=\frac{q\alpha_i}{2}
(I_n-\frac{\gamma}{N})^T
(I_n-\frac{\gamma}{N})+\frac{q\sum_{j=1,j\neq i}
^N\alpha_j}{2N^2}\gamma^T\gamma. 
\end{equation*}
The limiting population reduced cost is 
then
\begin{multline} \label{aux-cost-n}
J_{n,i}^{\infty}(u_{i},x^{(\infty)})=\\\ 
\mathbb{E} \Bigg (
\int_0^T \bigg\{ \frac{\alpha_iq}{2}
\|x_i\|^2 + q (x^{(\infty)})^{T} L_{\alpha_i} x_i 
+ \frac{\alpha_ir}{2} \|u_i\|^2 \bigg\} 
\mathrm{dt} \\ 
+\frac{\alpha_iM}{2} \min\limits_{j=1,\dots,l}\|
x_i(T)-p_j\|^2 \Bigg ). 
\end{multline}
where $L_{\alpha_i}=\bar{\alpha}
\gamma^T \gamma -\bar{\alpha}\gamma 
- \alpha_i\gamma^T$ and 
$\bar{\alpha}=\mathbb{E}\alpha_i$.

Noting the independence and identical distribution
of the initial states, weights and dynamic
parameters, we consider a generic agent 
with initial state $x^0$, dynamic parameters 
$\theta=(A_\theta,B_\theta)$ and weight $\alpha$.

We define $\Gamma^{\theta} 
\in C([0,T],\mathbb{R}^{n \times n})$, 
$\beta_k^{\theta \alpha} 
\in C([0,T],\mathbb{R}^n)$ and 
$\delta_k^{\theta \alpha} 
\in C([0,T],\mathbb{R})$
the unique solutions of the following backward 
propagating differential equations:
\begin{subequations}
\begin{align}
&\dot{\Gamma}^{\theta}-\frac{1}{r} 
\Gamma^{\theta}
 B_\theta B_\theta^{T}\Gamma^\theta 
+\Gamma^\theta A_\theta
+A_\theta^{T}\Gamma^\theta 
+q I_{n}=0  \label{eq:gamma-1-n} \\
&\dot{\beta}_k^{\theta \alpha}=\left(\frac{1}{r} 
\Gamma^\theta B_\theta B_\theta^{T}
-A_\theta^{T}\right )
\beta_k^{\theta \alpha} 
-q\frac{L_\alpha}{\alpha}
x^{(\infty)} \label{eq:beta-2-n} \\
&\dot{\delta}_k^{\theta \alpha}=\frac{1}{2r} 
(\beta_k^{\theta \alpha})^{T}
B_\theta B_\theta^{T}\beta_k^{\theta \alpha}
 -\frac{1}{2}q  
\Big\|\frac{L_\alpha}{\alpha}x^{(\infty)}
\Big \|^2,  \label{eq:delta-3-n} 
\end{align}
\end{subequations}
with the final conditions 
\[
\Gamma^\theta (T)=MI_{n}, \;\; 
\beta_k^{\theta \alpha} (T)=-Mp_k, 
\;\; \delta_k^{\theta \alpha} (T)=\frac{1}{2}M
 p_k^{T} p_k.\]

\begin{lem} \label{lemma:tracking-n}
The tracking problem (\ref{aux-cost-n}) has a unique 
optimal control law
\begin{align}\label{eq:ctr-n}
\hat{u}^{\theta \alpha}_{i}(t) = 
- \frac{1}{r} B_\theta^T \big 
(\Gamma^\theta(t) x_i + \beta^{\theta \alpha}_j(t)
 \big )
 && \text{if } x^0_i \in 
 D^{\theta \alpha}_j(x^{(\infty)}) 
\end{align}
where $\Gamma^{\theta}$, $\beta^{\theta \alpha}_j
$, $\delta^{\theta \alpha}_j$ are the unique 
solutions of (\ref{eq:gamma-1-n})-
(\ref{eq:delta-3-n}), and
\begin{multline} \label{eq:da-n}
D^{\theta \alpha}_j(x^{(\infty)}) =  \Big \{x\in 
\mathbb R^n 
\text{ such that}\\  
 \big (\beta^{\theta \alpha}_{j}(0)-\beta^{\theta
 \alpha}_{k}(0) 
 \big )^{T}
 x\leq \delta^{\theta \alpha}_{k}(0)
 -\delta^{\theta \alpha}_{j}(0), \, 
 \forall k=1,\dots,l \Big \}. 
\end{multline}
\end{lem}

==> app.tex <==
\appendices

\section{} \label{Proof1}

\subsection{Proof of Theorem \ref{reachability}}

    
% \subsection{Proof of Theorem \ref{lemma:existanceinit}}

% We use Schauder's fixed point theorem 
% \cite{FunAnaCon} to prove the existence 
% of a fixed point. We start by showing that 
% $G_\infty$ is a compact operator, that is, 
% continuous and maps bounded sets to 
% relatively compact sets.

% 1) \underline{Continuity}\\ 
% Let $x^{(\infty)}$ be in $C([0,T],\mathbb{R}
% ^n)$ and $\{x^{(\infty)}_k\}_{k\in 
% \mathbb{N}}$ 
% be a sequence converging to $x^{(\infty)}$ 
% in the Banach space $\big (C([0,T],\mathbb{R}
% ^n),\|.\|_\infty\big)$. 
% Let 
% \begin{multline*}
% Q_j=\|L\|+\max_{(\theta,t)\in \Theta \times [0,T]^2}\|\Phi_{\Pi_{j}^{\theta}}(t)\|\\
% +\max_{(\theta,t)\in \Theta \times [0,T]^4}\|\Psi_{j}^{\theta}(t)\|+\max\|M_{\theta j}\|
% +\max\|1/r_{\theta}\|.
% \end{multline*}
% We have
% \begin{multline*}
% \|G_\infty (x^{(\infty)}_k)-
% G_\infty (x^{(\infty)})\|_\infty \leq \\ 
% \sum_{j=1}^{l} Q_j \bigg \{V_{1j} +
% \Big(\|p_j\| T Q_j^2 + q \|x^{(\infty)}\|_\infty
% Q_j^2 T^2 \Big )V_{2j}\\
% + qQ_j^2T^2 \|x^{(\infty)}_k-x^{(\infty)}\|_
%  \infty \bigg \}, 
% \end{multline*}
% where
% \begin{align*}
% & V_{1j}=\int_\Theta \int_{\mathbb{R}^n}  
% \Big|\mathbbm{1}_{D^{\theta}_{j}(x^{(\infty)}
% _k)}(x^0)-\mathbbm{1}_{D^{\theta}_{j}
% (x^{(\infty)})}(x^0)\Big|\|x^0\| \, 
% \mathrm{d} \mathbb{P}_0\mathrm{d} \mathbb{P}_
% \theta\\
% & V_{2j}=\int_\Theta \int_{\mathbb{R}^n}  
% \Big|\mathbbm{1}_{D^{\theta}_{j}(x^{(\infty)}
% _k)}(x^0)-\mathbbm{1}_{D^{\theta}_{j}
% (x^{(\infty)})}(x^0)\Big| \, \mathrm{d} 
% \mathbb{P}_0\mathrm{d} \mathbb{P}_\theta.
% \end{align*} 
% Under Assumption \ref{assum-P0},
% \begin{align*}
% V_{1j}=\int_\Theta \int_{\mathbb{R}^n}  
% \Big|\mathbbm{1}_{\overset{\circ}{D}
% ^{\theta}_{j}(x^{(\infty)}
% _k)}(x^0)-\mathbbm{1}_{\overset{\circ}{D}
% ^{\theta}_{j}
% (x^{(\infty)})}(x^0)\Big|\|x^0\| \, 
% \mathrm{d} \mathbb{P}_0\mathrm{d} \mathbb{P}_
% \theta
% \end{align*} 
% But 
% \[\Big|\mathbbm{1}_{\overset{\circ}{D}
% ^{\theta}_{j}(x^{(\infty)}
% _k)}(x^0)-\mathbbm{1}_{\overset{\circ}{D}
% ^{\theta}_{j}
% (x^{(\infty)})}(x^0)\Big|\|x^0\| 
% \leq 2\|x^0\|\]
% and converges to zero for all $(x^0,\theta)$ 
% in $\mathbb{R}^n\times \Theta$. 
% Under Assumption \ref{assum-Ex2}, by Lebesgue's dominated convergence 
% theorem \cite{Rudin87_Real}, $V_{1j}$ 
% converges to zero.    
% By the same technique we prove that $V_{2j}$ 
% converges to zero. Hence, $G_\infty$ is 
% continuous. 

% 2) \underline{Compactness}\\
% Let $V$ be a bounded subset of $C([0,T],
% \mathbb{R}^n)$. 
% Let $\{G_\infty(x^{(\infty)}_k)\}_{k\in 
% \mathbb{N}} \in G_\infty(V)$.
% By the continuity of $\Phi_{\Pi_{j}^{\theta}}
% (\sigma,t)$ with respect to $(\sigma,t,
% \theta)$, 
% of its derivative with respect to $t$ and $
% \sigma$, and by the boundedness of $
% x^{(\infty)}_k$, 
% one can prove that for all $t, s$ in $[0,T]$, 
% \begin{equation*}
% \|G_\infty(x^{(\infty)}_k)(t)-G_
% \infty(x^{(\infty)}
% _k)(s)\|\leq \Big (K_1 \mathbb{E}\|x^0\| + 
% K_2 \Big ) |t-s|, 
% \end{equation*}
% where $K_1$ and $K_2$ are positive constants.   
% This inequality implies the uniform 
% boundedness and equicontinuity of 
% $\{G_\infty(x^{(\infty)}_k)\}_{k\in 
% \mathbb{N}}$. 
% By Arzela-Ascoli Theorem \cite{FunAnaCon}, 
% there exists a convergent subsequence of 
% $\{G_\infty(x^{(\infty)}_k)\}_{k\in 
% \mathbb{N}}$. 
% Hence, $G_\infty(V)$ and its closure are 
% compact sets and $G_\infty$ is a compact 
% operator. 
 
% 3) \underline{Existence of a fixed point}\\
% Having proved the compactness of $G_\infty$,  
% we now construct a nonempty, bounded, closed, 
% convex subset 
% $W \subset C([0,T],\mathbb{R}^n)$ such that 
% $G_\infty(W)\subset W$. The idea is to bound
% the right-hand side of (\ref{meaninit}) by
% a linear operator for which one can compute
% a fixed point $R(t)$. $W$ is then defined as the set of paths bounded by $R(t)$. Let
% \begin{equation*}
% Q=\sum_{j=1}^{l} \bigg \{ Q_j\mathbb{E}\|
% x^0\| +
% TQ_j^3\|p_j\|+qQ_j^3 \bigg \} . 
% \end{equation*}  
% We start by defining on $[0,T]$ the function
% \begin{align*}
% R(t)=\sum_{k=1}^{\infty}
% Q^k\int_0^t \! \ \int^T_{\tau_1} \! \dots \int_0^{\sigma_{k-1}} \! \ \int^T_{\tau_k} \! \  \, \mathrm{d}\sigma_k \mathrm{d}\tau_k \dots \mathrm{d}\sigma_1 \mathrm{d}\tau_{1}.
% \end{align*}
% $R$ is well defined (\cite[Lemma 3]
% {DBLP:journals/corr/SalhabMN15}). We define 
% the set 
% \[W=\Big \{x\in C([0,T],\mathbb{R}^n)|\, \|
% x(t)\| \leq R(t), \, \forall t\in [0,T]\Big 
% \}.\]
% $W$ is an nonempty, bounded, closed and 
% convex subset of $C([0,T],\mathbb{R}^n)$. $
% \forall x \in W$, $\forall t \in [0,T]$,
% \begin{equation*}
% \|G_\infty(x)(t)\| \leq Q+Q\int_{0}^{t} \; 
% \int^{T}_{\sigma} \; R(\tau) \, \mathrm{d}
% \tau \mathrm{d}\sigma = R(t).
% \end{equation*}
% Hence, $G_\infty(W)\subset W$. By Schauder's 
% Theorem, $G_\infty$ has a fixed point in 
% $W$.

\section{} \label{Proof2}

\subsection{Proof of Lemma \ref{appr}}



\subsection{Proof of Theorem \ref{th-optim}}


\section{} \label{Proof3}

\subsection{Proof of Lemma \ref{1-app}}



\subsection{Proof of Lemma \ref{2-app}}

 

\subsection{Proof of Theorem \ref{asym-cost-1}}


==> uniform.tex <==
\section{Uniform Population} \label{unif}
In this section, we analyze the uniform 
population, that is, the case where $
(A_i,B_i,r_i,M_{ij})=(A,B,r,M)
$ for all $i$. We derive an explicit 
form of the fixed point paths 
$x^{(\infty)}$. Moreover, we show that
the vector of fractions of players that
go towards each destination point is a fixed point
of a well defined map. 
In the following, we omit the 
index $\theta$ which is the same 
for all the agents.

We start by computing an explicit
form of the basins of attraction 
$D_j(x^{(\infty)})$ which are in case of
uniform population half planes delimited 
by hyperplanes. In fact, $\Gamma^\theta_
k$ defined in (\ref{eq:gamma-1-n}) and the related
functions, namely $\Pi_k^\theta$ and 
$\Phi_{\Pi_k^\theta}$ are the same for 
all the players
and are respectively denoted by $\Gamma$, $\Pi$ and 
$\Phi_{\Pi}$. Therefore, $\Gamma^
\theta_{jk}$ defined in (\ref{diff-1}) is equal 
to zero. 

By solving (\ref{eq:beta-2-n}) and
(\ref{eq:delta-3-n}) we obtain
\begin{equation} \label{eq:beta}
\begin{split}
&\beta_{k}(t)  =  -M\Phi_{\Pi}(t,T)
p_{k}- q \int_T^t \;  \Phi_{\Pi}(t,
\sigma)
Lx^{(\infty)}(\sigma) \, \mathrm{d}
\sigma  \\ 
&\delta_{k}(t)  =  \frac{1}{2}Mp_{k}^{T}
p_{k} \\ 
& +\frac{M^{2}}{2r}p_{k}^{T}\int_T^t \;  
\Psi(\eta,T,\eta,T) \, \mathrm{d}\eta 
\,p_{k}  \\  
&+\frac{Mq}{r}p_{k}^{T}\int_T^t \;  
\int_T^\eta \;  \Psi(\eta,T,\eta,
\sigma)Lx^{(\infty)}(\sigma) \, 
\mathrm{d}\sigma \mathrm{d}\eta \\
&+ \frac{q^{2}}{2r}\int_T^t 
\int_T^\eta \int_T^\eta
(x^{(\infty)})^{T}(\sigma)L
\Psi(\eta,\sigma,\eta,\tau)Lx^{(\infty)}
(\tau) 
\,  \mathrm{d}\tau \mathrm{d}\sigma 
\mathrm{d}\eta. 
\end{split}
\end{equation}
By replacing (\ref{eq:beta}) in 
the expression of $D_j(x^{(\infty)})$, 
(\ref{eq:da}) can be written
\begin{multline} \label{eq:dae}
D_j(x^{(\infty)}) = \Big \{ x\in \mathbb R^n 
\text{ such that}\\ (\beta_{jk})^{T}x \leq 
\delta_{jk}^{(1)} + \delta_{jk}^{(2)}
(x^{(\infty)}),\, \forall k=1,\dots,l \Big \} 
\end{multline}
where
\begin{equation} \label{eq:de0}
\begin{split}
\beta_{jk} & = M\Phi_{\Pi}(0,T)(p_{k}-p_{j})\\
\delta^{(1)}_{jk} & = 
\frac{1}{2}Mp_{k}^{T}p_{k}-\frac{1}{2}Mp_{j}^{T}p_{j} \\
&+\frac{M^{2}}{2r}p_{k}^{T} \int_T^0 \;  
\Psi(\eta,T,\eta,T) \, \mathrm{d}\eta \,p_{k}\\ 
&-\frac{M^{2}}{2r}p_{j}^{T} \int_T^0 \;  
\Psi(\eta,T,\eta,T) \, \mathrm{d}\eta \,p_{j} \\
\delta^{(2)}_{jk}(\hat{\bar{x}})&  =
\frac{Mq}{r}(p_{k}-p_{j})^{T} \times \\
&\int_T^0 \! \int_T^\eta \;  
\Psi(\eta,T,\eta,\sigma)Lx^{(\infty)}(\sigma) 
\, \mathrm{d}\sigma \mathrm{d}\eta. 
\end{split} 
\end{equation}

The map $G_\infty$ defined in (\ref{meaninit}) reduces to
\begin{multline} \label{eq:Mean-Mean}
 \bar{x}_\infty  = \mathbb{E} \hat{x}_0
  = G_\infty (x^{(\infty)}) = 
\Phi_{\Pi}^{T}(0,t) \mu_0 +\\
\sum_{j=1}^l\mathbb{P}_0(D_j(x^{(\infty)})\frac{M}{r}
\int_0^t \! \ \Psi(\sigma,t,\sigma,T)
p_{j} \, \mathrm{d}\sigma \\
 +\frac{q}{r}\int_0^t \! \ \int_T^\sigma 
 \! \ \Psi(\sigma,t,\sigma,\tau)Lx^{(\infty)}
 (\tau) \, \mathrm{d}\tau \mathrm{d}\sigma 
\end{multline}
where $\mu_0=\mathbb{E} x^0$.

We define $R_{1}(t)=\Phi_{\Pi}^{T}(0,t)
\tilde{R}_1(t)$, $R_{2}(t)=\Phi_{\Pi}
^{T}(0,t)\tilde{R}_2(t)$ where $
\tilde{R}_1$ and $\tilde{R}_2$, the unique solutions of
\begin{equation} \label{eq:r1r2}
\begin{split}
\dot{\tilde{R}}_1&=\frac{q}{r}\int_T^t \; 
\Psi(t,0,t,\sigma)L
\Phi_{\Pi}^{T}(0,\sigma)\tilde{R}_1(\sigma)
  \, \mathrm{d}\sigma \\
\dot{\tilde{R}}_2&=\frac{q}{r}\int_T^t \; 
\Psi(t,0,t,\sigma)L
\Phi_{\Pi}^{T}(0,\sigma)\tilde{R}_2(\sigma)
  \, \mathrm{d}\sigma \\
&+\frac{M}{r}\Psi(t,0,t,T)
\end{split}
\end{equation}
with initial conditions $\tilde{R}_1(0)=
I_n, \; \tilde{R}_2(0)=0$. We define
\begin{align} \label{theta1}
\theta_{jk}^{(1)}=&\frac{Mq}{r}
(p_{k}^{T}-p_{j}^{T})
\int_T^0 \!  \ \int_T^\eta \! 
\Psi(\eta,T,\eta,\sigma)LR_{1}(\sigma)
 \, \mathrm{d}\sigma \mathrm{d}\eta 
 \nonumber\\
  =&M(p_j^T-p_k^T) \big (R_1(T)-\Phi_{\Pi}^T(0,T)\big)
\end{align}
\begin{align} \label{theta2}
&\theta_{jk}^{(2)}=\frac{Mq}{r}
(p_{k}^{T}-p_{j}^{T})
\int_T^0 \!  \ \int_T^\eta \! 
\Psi(\eta,T,\eta,\sigma)LR_{2}(\sigma)
 \, \mathrm{d}\sigma \mathrm{d}\eta
 \nonumber \\
 &= M(p_j^T-p_k^T) \bigg (R_2(T)-\frac{M}{r} \int^T_0 \, \Psi (\eta,T,\eta,T) \, \mathrm{d}\eta\bigg).
\end{align} 

We define a map $F_\infty$ from $[0,T]^l$ into 
itself such that 
\begin{multline*}
F_\infty(\lambda_1,\dots,\lambda_l)=\\
 \begin{bmatrix}
\mathbb{P}\Big ((\beta_{1j})^Tx^0 
\leq \delta^{(1)}_{1j} + \theta^{(1)}_{1j}\mu_{0} 
+ \theta^{(2)}_{1j}p_\lambda,\, 
\forall j=1,\dots,l\Big)\\
\vdots\\
\mathbb{P}\Big ((\beta_{lj})^Tx^0 
\leq \delta^{(1)}_{lj} + \theta^{(1)}_{lj}
\mu_{0} + \theta^{(2)}_{lj}p_\lambda,\, 
\forall j=1,\dots,l\Big) 
\end{bmatrix}^T
\end{multline*}
where $p_\lambda=\sum_{j=1}^l \lambda_j p_j$.
Noting the new form of the basins of 
attraction, a weaker assumption than
Assumption \ref{assum-P0} is sufficient
to prove the existence of a fixed point.

\begin{assum} \label{assum-P0-1}
We assume that $\mathbb{P}_0$
is such that the $\mathbbm{P}_0-$measure of hyperplanes is zero.
\end{assum}
\begin{thm} \label{lemma:existance11}
Under Assumption \ref{assum-P0-1}, the following statements hold 
\begin{enumerate}
\item $x^{(\infty)}$ is a fixed point of 
$G_\infty$ if and only if there exists 
$\lambda=(\lambda_1,\dots,\lambda_l)$ in $[0,1]^l$ 
such that 
\begin{align}\label{stineq-multi}
F_\infty(\lambda)=\lambda
\end{align} 
for 
\begin{equation} \label{fixed-point}
x^{(\infty)}(t)=
R_1(t)\mu_0+R_2(t)p_\lambda.
\end{equation} 
\item $F_\infty$ has a fixed point 
(equivalently $G_\infty$ has a fixed point).
\end{enumerate}
\end{thm}
\begin{IEEEproof}
See
\cite[Theorem 6]{DBLP:journals/corr/SalhabMN15}.
\end{IEEEproof}

Theorem \ref{lemma:existance11} 
establishes 
a one to one map between the
potential (infinite population) 
macroscopic behaviors ($x^{(\infty)}$) 
and the fixed points $\lambda$ of an 
operator 
$F_\infty$ defined on a finite 
dimensional space. The $j$-th 
coordinate of a fixed point
$\lambda$ is the fraction of players (in a infinite size population) that goes
towards $p_j$.

Thus, given the initial distribution
$\mathbb{P}_0$, the players compute,
prior moving, 
a fixed point $\lambda$ of 
(\ref{stineq-multi}) and the 
corresponding fixed point path
(\ref{fixed-point}). Once $x^{(\infty)}$
is computed, the agents start moving 
by applying the optimal control laws
(\ref{eq:ctr}). For the computation of 
a fixed point of $F_\infty$ one can 
refer to \cite{DBLP:journals/corr/
SalhabMN15}.   

Following Theorem \ref{asym-cost-1},
the asymptotic optimal social cost
for a uniform population can be 
written
\begin{align*}
&\lim\limits_{N \rightarrow \infty}
\inf\limits_{u \in U^N} 
\frac{1}{N}J_{soc}(u,x^{(N)})=
\sum_{j=1}^l 
\int  \mathbbm{1}_{D_{j}
(x^{(\infty)})}
(x^0) \times\\
&\Big\{ 
\frac{1}{2}(x^0)^T \Gamma (0) x^0
+(\beta_j (0))^T x^0 + 
\delta_j (0) \Big \} \mathrm{d} \mathbb{P}_0\\
 &-\frac{1}{2}\int_0^T q
(x^{(\infty)})^T Lx^{(\infty)} \mathrm{dt}\\
&=-\frac{1}{2}\int_0^T q
(x^{(\infty)})^T Lx^{(\infty)} \mathrm{dt}
+\frac{1}{2}\mathrm{Tr}\Big(\Gamma \mathbb{E}\big(x^0(x^0)^T\big)\Big)\\
&+\sum_{j=1}^l \Big \{ 
(\beta_j (0))^T\mathbb{E}\Big(x^0;D_{j}
(x^{(\infty)})\Big)+\delta_j (0)
\mathbb{P}_0\Big(D_{j}
(x^{(\infty)})\Big) \Big \}.
\end{align*}
